Xapagy: a cognitive architecture for narrative reasoning

We introduce the Xapagy cognitive architecture: a software system designed to perform narrative reasoning. The architecture has been designed from scratch to model and mimic the activities performed by humans when witnessing, reading, recalling, narrating and talking about stories.

==> Conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusions}

The Xapagy system is an active software project, in development since 2008. It has been designed to perform narrative reasoning, that is, to mimic the human behavior when reasoning about stories. The objective of this paper was to convey the architecture of the system, with an emphasis on the design decisions which differentiate it from its peers from the artificial intelligence literature. 

In order to fit the description of the architecture in a single paper, we had to omit certain details. For instance, the spike activities and diffusion activities which maintain the shadows and headless shadows have been presented in an informal manner. The various narrative reasoning modalities outlines in Section~\ref{sec:NarrativeReasoning} would deserve separate and extensive treatment, which will be provided in future papers. 



==> RelatedWork.tex <==
\section{Related work}
\label{sec:RelatedWork}

The Xapagy system had been developed from scratch but not in a void. In the following we shall compare and contrast it against a small collection of representative systems. Most of these systems represent bodies of work which fit the Newell definition of cognitive architecture~\cite{Newell-1994-Unified} as integrative systems which try to provide a model of a large subset of the human cognition even if they do not answer to all the twelve requirements of a human cognitive architecture as proposed in the ``Newell test'' (Anderson and Lebiere \cite{AndersonLebiere-2003-NewellTest}). Some of them have not been explicitly positioned as cognitive architectures. 

We shall look both at differences and similarities in the approach. The Xapagy system has taken a somewhat unusual approach to issues such as instance and concept as well as in focusing on episodic memory and shadowing as a single reasoning model. These choices have their root in the application, computational efficiency considerations - but also in the desire to try out roads less traveled. Despite of this, we found unexpected similarities and convergencies between Xapagy and approaches which have started out with radically different assumptions. 

Xapagy is a new system, developed over the last three years and first described in this paper. When comparing it against other architectures we will also focus not only on what we learned from some of these systems but also what we might learn in the future. 

% *********************************************************
%
%  ACT-R
%
% *********************************************************

\subsection*{The ACT-R cognitive architecture}

ACT-R (Anderson and Lebiere \cite{Anderson-1998-AtomicComponentsOfThought}, Anderson et al. \cite{Anderson-2004-IntegratedTheoryOfMind}) is a cognitive architecture developed based on the theoretical models of John R. Anderson. It is the center of an active community of researchers with many variants adapted to perform specific tasks. Overall, the ACT-R community has been eager to integrate the system with external models. Earlier extensions, such as the ACT-R/PM (perceptual-motor) model have been integrated into the core of the ACT-R system. A recent integration effort created the SAL hybrid architecture through the integration of ACT-R and the Leabra neural model (Jilk et al. \cite{Jilk-2008-SAL}). 

The central idea of the ACT-R system is the use of the {\em production} as the model of the functioning of the human brain. A production requires some preconditions to be satisfied, and then it can ``fire'', performing a certain action. Unlike other models such as EPIC, ACT-R is based on a serial-bottleneck theory of cognition, where only  one production can fire at a time. This is similar to the Xapagy system which also allows only one verb instance to be inserted into the focus at a time. Although the idea of a production is a computer science term, it has been found that it can be quite efficiently mapped to lower level terms, connectionist systems and even biological brain functions. 

The flow of cognition in ACT-R happens through the system choosing productions based on its current {\em buffers} (largely equivalent to the Xapagy focus or the working memory in several other systems). The buffers can hold the current goal, its declarative memory, perceptual and motor modules, where it goes through the matching /selection / execution model.

ACT-R is a goal oriented system, it describes the active behavior of an agent. In general, ACT-R emphasizes the conceptual knowledge as encoded in the productions, and it does not focus on the episodic knowledge. 

In contrast, for the Xapagy system, the episodic knowledge is the main focus. This is not really a choice, when we consider the fact that the objective of the Xapagy system is is the reasoning about stories. 


% *********************************************************
%
%  The SOAR cognitive architecture
%
% *********************************************************

\subsection*{The SOAR cognitive architecture}

SOAR is a cognitive architecture with an active academic community and history of successful commercial application. In its initial version (Laird, Newell and Rosenbloom \cite{Laird-1987-Soar}) SOAR was primarily a symbolic production system. However, its recent development path increasingly integrates non-symbolic memory and processing components in the architecture (Laird \cite{Laird-2008-ExtendingSoar}).

In its traditional version, SOAR has a long term memory (encoded as production rules) and a short term memory (encoded as a symbolic graph structure where objects are represented with properties and relations). The SOAR system performs cognition by matching and firing production rules. SOAR modulates the choice of the production to fire through operators. If the current preferences are insufficient for the choice of the production rule to fire, the SOAR system declares an {\em impasse}, automatically creating a new sub-state with the explicit goal to resolve it. This can be performed repeatedly and recursively, leading to an automatic meta-reasoning structure. 

The recent version of the SOAR system extends the system in form of non-symbolic knowledge representations (and the implied memory and processing modules) as well as new learning models for knowledge not easily encodable in form of rules.

From the point of view of the relationship to the Xapagy system it is important that the new version of SOAR implements episodic memory in form of temporally ordered snapshots of working memory. Recorded episodes can be retrieved by the creation of a {\em cue} which is the partial specification of a working memory. The retrieved episodes are stored in a special buffer, the exact recall of a sequence of episodes is possible. The retrieval of episodes is also affected by a new module modeling the activation level of working memory. 

Compared with the Xapagy architecture, the main difference is, again, the emphasis on the episodic memory placed by the Xapagy system. SOAR defines several memory models (procedural knowledge encoded as rules, semantic memory (facts about the world) with the episodic memory being a relatively recent addition. In contrast the episodic memory is essentially the only memory model in Xapagy\footnote{Xapagy also defines conceptual and dictionary knowledge. Conceptual knowledge is implicitly present in SOAR (and basically all the other cognitive architectures, even if they do not appear a separate module). Dictionary knowledge is also necessarily present in any system which uses some kind of external language.}. 

The cue and working memory based episodic memory retrieval parallels the Xapagy's continuation HLS model. There is however a major difference in what the actual recall does. In SOAR it is possible to accurately recall a previous episode, with the complete snapshot of the working memory. In Xapagy this is impossible - it is not sure that even the general outline of the recalled story will be accurately recreated (see Section~\ref{sec:StoryCreation}).


% *********************************************************
%
%  The ICARUS cognitive architecture
%
% *********************************************************
\subsection*{The ICARUS cognitive architecture}

The ICARUS system (Langley and Choi \cite{Langley-2006-ICARUS}) is a cognitive architecture which focuses on cognition occurring in the physical context. Its cognitive behavior cycle is strongly tied to the perceptual input from the environment, with the mental structures grounded in the perception and the actions of the agent. ICARUS models  {\em concepts} and {\em skills} as encoding different aspects of knowledge, memorized as different cognitive structures. It assumes that each element of the short term memory has a corresponding generalized structure in the hierarchically organized long term memory. 

Comparing ICARUS and Xapagy is difficult, as the physical, grounded orientation of ICARUS and the story oriented application domain of Xapagy have very little overlap. Inevitably, however, Xapagy needs to extend towards application scenarios where the stories are recorded as an active participant in the events (rather than as a more or less passive observer of events or listener of narrated stories). Thus the ICARUS system can serve as inspiration for future Xapagy extensions for embodied action and goal directed reasoning. 

% *********************************************************
%
%  The Polyscheme cognitive architecture
%
% *********************************************************
\subsection*{The Polyscheme cognitive architecture}

The Polyscheme system (Cassimatis et al. \cite{Cassimatis-2004-Integrating}) is a cognitive architecture designed to integrate multiple different representations and reasoning algorithms. Polyscheme reasoning proceeds through sequential mental simulations where the different cognitive reasoning and planning models are encapsulated in {\em specialist} modules. The architecture allows even purely reactive components to react to simulated states of the world, thus integrating reasoning and planning with perception and action. 

The integration of the different specialists is performed through a common communication language, used to translate information between specialists. Beyond this, however, each specialist can use its own internal data representations. 

The Polyscheme system implements a rigorous and consistent way to annotate states as being in the past, hypothetical, distant or invisible. 

There are apparently irreconcilable differences between the architectural approach of Polyscheme and Xapagy. Polyscheme is fundamentally built on the integration of multiple representations and reasoning models while Xapagy uses a single representation and a shadowing as a single reasoning model. 

A closer look, however, also finds many parallels. The common language used between specialist modules can be seen as an analogue to the Xapagy verb instance representation. 

Many of the specialist modules in Polyscheme would need to be also implemented outside the shadow/HLS reasoning model if Xapagy would be used in their application domain. For instance in the Polybot robot application one of the specialists identifies the location and category of the objects using color segmentation. This obviously cannot be implemented through shadowing - should the Xapagy system ever be controlling a robot, the solution would roughly be the same: a specialized visual module which communicates with the rest of the system by inserting instances and verb instances into the focus. 

Finally, the shadow/HLS mechanism in Xapagy can be considered a type of simulation of recent events based on past knowledge, which is a close parallel to what the Polyscheme simulation model does.  

% *********************************************************
%
%  The EPIC cognitive architecture
%
% *********************************************************

\subsection*{The EPIC cognitive architecture}

The EPIC cognitive architecture (Kieras and Meyer \cite{Kieras-1997-EPIC}) has been implemented with the explicit goal to model the human multimodal and multiple task performance. The EPIC architecture's goal is to understand and model human behavior (preferably, through a predictive model) rather than to create an artificially intelligent agent. 

As ACT-R and SOAR, EPIC is a production based system. One of the influential differences of the EPIC system is that it does not assume a serialized bottleneck on the firing of the productions. However, the number of productions which can be actually be instantiated simultaneously is limited by resource limitations, for instance the various components of the working memory, the processing speed, and the physical limitations of sensors and actuators (eyes can focus on one point at a time, hands can grab a single object, and so on). 

What the Xapagy system can learn from EPIC is the lesson which many other architectures have also drawn - that is, that the perceived serialization of some aspects of human behavior can occur naturally - they need not be enforced through artificial constraints. 


% *********************************************************
%
%  CLARION cognitive architecture
%
% *********************************************************

\subsection*{The CLARION cognitive architecture}

The stated goal of the CLARION architecture (Sun \cite{Sun-2006-CLARION}) is to capture cognitive modeling aspects not adequately addressed by other cognitive architectures: the implicit-explicit interaction, the cognitive-metacognitive interaction and the cognitive-motivational interaction.

Overall, CLARION is an integrative model with separate functional subsystems (such as the action centered, metacognitive and motivational subsystem). Each subsystem has a has a dual representational structure, separately for implicit and explicit representations. This separation of the high level (symbolic, explicit) and low level (non-symbolic, implicit) representations is consistently carried through throughout the architecture. These two representation models are independently operating and compete for the right to perform an action through well defined interaction models. For instance, the system contains models for learning symbolic rules from subsymbolic information. The CLARION system also contains built-in motivational and metacognitive constructs. 

On a superficial look, there appears to be very little similarity between CLARION and Xapagy. CLARION's characteristic is that its architecture explicitly models several dichotomies of human cognition (explicit vs. implicit, action vs. deliberation, symbolic vs. subsymbolic). If one wishes to identify where a certain human reasoning ability is modeled, a single look at the CLARION's architectural diagram can point to the component responsible. In contrast, Xapagy uses a single reasoning model, shadowing, and whatever dichotomies must appear in the external behavior, it must emerge from a unique internal model. 

Yet, despite the very different architecture, a careful comparison study can find that parallels between the turn architectures can be drawn. For instance, CLARION uses a mix of similarity based and rule-based reasonings - these components can be mapped to the various shadow maintenance activities which deploy a mix of structural and similarity based matching techniques. 

% *********************************************************
%
%  The KARMA story understanding system and related work
%
% *********************************************************

\subsection*{The KARMA story understanding system and related work}

The KARMA system for story understanding (Narayanan \cite{Narayanan-1997-Thesis}) had demonstrated the understanding of simple stories and narrative fragments in the domain of international politics and economics as described in journalism.

One feature of the system is the ability to represent, reason about, and understand metaphors which present abstract concepts (such as those in international politics and economy), in terms of the physical motion, forces, terrain features. It uses the Event Structure Metaphor that projects inferences from physical motion and manipulation to abstract actions, goals and policies. 

From the point of view of practical implementation, the KARMA system uses a model called {\em x-schemas} which are parametrized routines, with internal state which execute when invoked. They are implemented as an extension to Petri-nets (to allow run-time binding, hierarchical action sets and stochastic transitions).

% Another interesting component is the approach which Narayanan gives to counterfactuals, based on a simulation semantics (Narayanan: Mind changes). 

The KARMA system is strongly focused on the study of {\em aspect} the study of linguistic devices which profile and focus on the internal temporal character of the event. 

A recent paper (Lakoff and Narayanan \cite{Lakoff-2010-ComputationalModelOfNarrative})  described a roadmap towards a system which understand human narratives by exploiting the cognitive structures of human motivations, goals, actions, events and outcomes. The authors outline a number of directions towards which future narrative systems need to work, and order them in {\em dimensions of narrative structure}: the moral system of the narrative (stories as guides to living), folk theories of how people and things work, overall plot structures (these are in many way resemble summarizations in Xapagy), plot schemas, motif structures, and narrative variations. 

% *********************************************************
%
%  Computational models of the narrative
%
% *********************************************************

%\subsection{Computational models of the narrative}
%\label{sec:RWComputationalNarrative}


% *********************************************************
%
%  E.T. Mueller's work on daydreaming
%
% *********************************************************

\subsection*{The DAYDREAMER system}

The DAYDREAMER system (Mueller and Dyer \cite{Mueller-1985-TowardsDaydreaming}) was a system which generated stories, based on, and initiated from actual experiences. The system used in the guidance of these story creations four goals which were identified as frequently appearing in daydreaming: rationalization, revenge, failure/success reversal (exploration of alternatives), and preparation (generation of hypothetical future scenarios). 

DAYDREAMER had been strongly tied to models of emotion: defined notions of success of a goal (which produces a positive emotion) and failure (producing negative emotion). It proposed that the basic mechanism for scenario generation is plannning. 

The DAYDREAMER system was taking a similar approach to Xapagy in the fact that both the actual experiences and the daydreamed experiences are equally available to recall. 

DAYDREAMER modeled a dynamic episodic memory (Tulving \cite{Tulving-1972-EpisodicAndSemantic}, Schank \cite{schank1982dynamic}), constantly modified during daydreaming. In Xapagy, the episodic memory is not, in fact, modified, yet the practical impact is similar, as the way in which the recall happens through self-shadowing, it creates a behavior compatible with a dynamic memory for the external observer. 

% *********************************************************
%
%  Leon and Garvas
%
% *********************************************************

% \subsubsection{Leon and Garvas in Madrid}


% *********************************************************
%
%  Chalmers and Jurafsky
%
% *********************************************************

\subsection*{Recent work on narrative schemas by Chalmers and Jurafski}

An body of work, with a high relevance to the Xapagy system has been recently reported by Chambers and Jurafsky \cite{Chambers-2008-NarrativeEventChains, Chambers-2009-NarrativeSchemasParticipants}. The work centers on the learning of narrative schemas, which they define as coherent sequences or sets of events with participants who are defined as semantic roles, which can be fitted by appropriate persons. 

This work can bee seen as a restart of the semantic NLP tradition of the 1970 and 80s, which used representations such as scripts (Shank and Abelson \cite{Schank-1977-Scripts}). This research direction had become marginalized in the 1990's as the knowledge engineering requirements appeared to be overwhelming. The work of Chalmers and Jurafski promises to reboot this research direction as the narrative schemas can be inferred or learned in an unsupervised way from raw input.

In \cite{Chambers-2008-NarrativeEventChains, Chambers-2009-NarrativeSchemasParticipants} successfully show scema and role inference, starting from preprocessed natural language. The evaluate the system using the {\em narrative cloze} test, an variation of the classical word-based cloze test, where an event is removed from a known narrative chain, and the system needs to infer the missing event. 

The work is very close to the Xapagy system in its external objectives, as well as in some of the details of the processes (e.g. some of the shadow maintenance DAs are close relatives of the algorithms used by the authors). It is true, Chambers and Jurafsky start from English text, not pidgin, but they are using independent preprocessing algorithms to resolve the references (albeit with some level of uncertainty). Practically, the input of the algorithms is closely related to the verb instance form of the Xapagy input. 

There is, however, a difference between the two approaches, which, depending on how we look at it, is either a major philosophical difference or an implementation detail. The assumption of Chambers and Jurafsky is that {\em scripts physically exist}, that the agents have an explicit data structure, which is, let us say, the restaurant schema, which is the subject of knowledge engineering or learning.

In contrast, in Xapagy, such an internal scheme does not exist as an explicit data structure. The reasoning model of Xapagy (shadows and headless shadows) do not create permanent intermediary structures: reasoning always starts with the concrete, originally memorized story lines. 

Looking from another perspective, however, the differences are not as great. For instance, a Xapagy agent, asked to confabulate a restaurant scene based on generic participants, will recall the same sequence as the one which one would obtained from a narrative schema initialized with the same participants in the specific roles. So, for an external observer, which sees the system's behavior but not the internal structure, these systems would be hard to distinguish (at least as long as we consider typical scenarios - for atypical scenarios, exceptions and borderline cases there is a larger freedom of movement for both systems). 


